Diffusion Model Compression for Image-to-Image Translation

As recent advances in large-scale Text-to-Image (T2I) diffusion models have yielded remarkable high-quality image generation, diverse downstream Image-to-Image (I2I) applications have emerged. Despite the impressive results achieved by these I2I models, their practical utility is hampered by their large model size and the computational burden of the iterative denoising process. In this paper, we propose a novel compression method tailored for diffusion-based I2I models. Based on the observations that the image conditions of I2I models already provide rich information on image structures, and that the time steps with a larger impact tend to be biased, we develop surprisingly simple yet effective approaches for reducing the model size and latency. We validate the effectiveness of our method on three representative I2I tasks: InstructPix2Pix for image editing, StableSR for image restoration, and ControlNet for image-conditional image generation. Our approach achieves satisfactory output quality with 39.2%, 56.4% and 39.2% reduction in model footprint, as well as 81.4%, 68.7% and 31.1% decrease in latency to InstructPix2Pix, StableSR and ControlNet, respectively.

==> figs/app.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{assets/app.pdf}
  \vspace{-2mm}
  \caption{Applications of our method to other downstream tasks}
  \label{fig:app}
  \vspace{-5mm}
\end{figure}



==> figs/autodiff-ip2p-quant.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\columnwidth]{assets/autodiff-ip2p-quant.pdf}
  \caption{}
  \label{fig:autodiff-ip2p-quant}
\end{figure}


==> figs/autodiff-layer.tex <==
\begin{minipage}{\textwidth}
  \hspace{-7mm}
  \begin{minipage}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{assets/autodiff-skip.pdf}
    % \vspace{-3mm}
    \captionof{figure}{Layer-skip results of AutoDiffusion. The colored dots indicate the layers that are skipped at each time step. A layer to be removed must be selected across all time steps. They fail to remove layers.}
    \label{fig:layer-skip}
  \strut\end{minipage} %
  % \hfill\allowbreak
  % \hfill
  \hspace{+3mm}
  \begin{minipage}[b]{0.45\textwidth}
    \centering
    \scalebox{0.70}{
            \begin{tabular}{cccccc}
            \Xhline{2\arrayrulewidth}
            \multicolumn{1}{l}{}                                                        & Step & T.O.    & + Skip   & $\Delta$ & $\Delta$Time \\ \hline\hline
            \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Instruct-\\ Pix2Pix~\cite{ip2p}\end{tabular}} & 5    & 20.64 & 20.64 & 0.00     & 0.0\%        \\
                                                                                        & 10   & 24.79 & 24.61 & -0.18    & 0.2\%        \\ \hline
            \multirow{2}{*}{StableSR~\cite{stablesr}}                                                   & 5    & 26.58 & 26.23 & -0.35    & 2.7\%        \\
                                                                                        & 10   & 29.03 & 27.80 & -1.23    & 2.8\%        \\
            \Xhline{2\arrayrulewidth}
            \end{tabular}
      }
      \captionof{table}{
      ``T.O'' and ``+Skip'' indicate the PSNR metrics for the time-step optimization and network skipping of AutoDiffusion. ``$\Delta$'' and ``$\Delta$Time'' represent PSNR and latency reduction after layer-skip.
      }
    \label{tbl:layer-skip} 
  \strut\end{minipage}
  \vspace{-3mm}
\end{minipage}

==> figs/bksdm.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.66\linewidth}
         \centering
         \includegraphics[width=0.95\linewidth]{assets/bksdm-qual.pdf}
         \caption{Qualitative comparisons}
         \label{fig:quant-fig-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         % \includegraphics[width=1.0\linewidth,height=4.5cm]{example-image-duck}
         \includegraphics[width=1.0\linewidth]{assets/bksdm-quant.pdf}
         \caption{Quantitative comparisons}
         \label{fig:quant-fig-b}
     \end{subfigure}
    \vspace{-5mm}
        \caption{Comparisons with BK-SDM~\cite{bksdm} and our depth-skip compression to InstructPix2Pix~\cite{ip2p}. These demonstrate that our approach produces higher-quality image editing results with a smaller model size. \rt{Removed}}
        \label{fig:bksdm-ip2p}
        \vspace{-5mm}
\end{figure}

==> figs/diff-pruning.tex <==
\begin{figure}[t]
     \centering
   \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1.0\linewidth]{assets/diff-pruning-quant.pdf}
         \caption{Quantitative comparison}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.67\linewidth}
         \centering
         \includegraphics[width=1.0\linewidth]{assets/diff-pruning-qual.pdf}
         \caption{Qualitative comparison}
     \end{subfigure}
    
    \vspace{-0mm}
        \caption{Qualitative and quantitative comparisons for various configurations where depth-skip compression combined with Diff-pruning~\cite{diffpruning} is applied to IP2P~\cite{ip2p}.
        D9 refers to the application of depth-skip compression at the 9th depth level. The percentage indicates the model size relative to the original. }
        \label{fig:diffprung}
        \vspace{-0mm}
\end{figure}

==> figs/ip2p-depthskip-qual.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/ip2p-depthskip-qual.pdf}
  \caption{\kkw{Describe caption}}
  \label{fig:ip2p-ds-qual}
\end{figure}


==> figs/ip2p-depthskip.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/depthskip-ip2p.pdf}
  \caption{\kkw{Describe caption}}
  \label{fig:depthskip-ip2p}
\end{figure}



==> figs/ip2p-ds-quant.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{assets/ip2p-ds-quant.pdf}
  \caption{
Trade-off between consistency of input image and editing for various depth-skip configurations applied to IP2P~\cite{ip2p}.
  }
  \label{fig:ip2p-ds-quant}
  \vspace{-3mm}
\end{figure}



==> figs/multi-depth-base.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\columnwidth]{assets/baseline-ip2p.pdf}
  \caption{...}
  \label{fig:muli-depth-baseline}
\end{figure}


==> figs/multi-depth-cmp.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\columnwidth]{assets/multidepth-ip2p.pdf}
  \caption{}
  \label{fig:muli-depth-cmp}
\end{figure}


==> figs/qual_cmp.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{assets/qual_cmp.pdf}
  \caption{...}
  \label{fig:d6}
\end{figure*}

==> figs/sdsr-ds.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/sdsr-ds.pdf}
  \caption{\kkw{This is final}}
  \label{fig:sdsr-ds}
\end{figure}



==> figs/time-quant.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/time-quant.pdf}
  \vspace{-7mm}
  \caption{
  We plot speeds to reach comparable PSNR with original sample for uniform timestep and ours. For all cases, we achieve same PSNR faster than uniform timestep.}
  \label{fig:time-quant}
  \vspace{-3mm}
\end{figure}


==> figs/timeskip.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/timeskip.pdf}
  \caption{\kkw{The actual values should be changed}}
  \label{fig:timeskip}
\end{figure}



==> tbls/_obsolete-autodiff-copy.tex <==
\begin{table}[]
\centering

\scalebox{1}{
\begin{tabular}{cccccc}

\Xhline{2\arrayrulewidth}
\multicolumn{2}{l}{\multirow{2}{*}{\textbf{}}} & \multicolumn{2}{c}{5 step} & \multicolumn{2}{c}{10step} \\
\multicolumn{2}{l}{}                           & PSNR        &  Skip        & PSNR       &  Skip      \\ \hline\hline
\multirow{2}{*}{IP2P}        & AutoDiff        & 20.64       & 0            & 24.61      & 2             \\
                             & Ours            & 0.00        & N            & 0.00       & N             \\ \hline
\multirow{2}{*}{StableSR}    & AutoDiff        & 26.23       & 7            & 27.80      & 15            \\
                             & Ours            & 0.00        & N            & 0.00       & N             \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\kkw{WIP}}
\end{table}


==> tbls/_obsolete-autodiff.tex <==
\begin{table*}[t]
\centering

\scalebox{0.88}{

\begin{tabular}{cccccccc}

\Xhline{2\arrayrulewidth}
\multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{3}{c}{5 step}                               & \multicolumn{3}{c}{10 step}                              \\
\multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & Timestep    & Timestep + Layer      & Acceleration   & Timestep      & Timestep + Layer     & Acceleration        \\ \hline\hline
\multirow{2}{*}{InstructPix2Pix~\cite{ip2p}}     & AutoDiffusion~\cite{autodiff}        & 20.643          & 20.643           & X           & 24.791          & 24.609           & X           \\
                          & Ours                 & \textbf{21.999} & \textbf{21.409} & \textbf{X}  & \textbf{25.856} & \textbf{25.269} & \textbf{16} \\ \hline
\multirow{2}{*}{StableSR~\cite{stablesr}} & AutoDiffusion~\cite{autodiff}        & 26.581          & 26.228           & X           & 29.027          & 27.801           & X          \\
                          & Ours                 & \textbf{27.456} & \textbf{26.849}  & \textbf{X} & \textbf{32.461} & \textbf{30.611}  & \textbf{X} \\
\Xhline{2\arrayrulewidth}
\end{tabular}

}
\caption{Quantitative comparison with AutoDiffusion~\cite{autodiff}. The "Timestep" and "Timestep + Layer" columns indicate the PSNR results for the timestep optimization and additional network skipping, respectively. The "Acceleration" column shows the improvement in inference speed. Our method outperforms in both timestep and joint optimization, achieving faster inference and higher accuracy.}
\label{tbl:autodiff}
\end{table*}


==> tbls/_obsolete-sdsr-ds.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{

\begin{tabular}{lrrrrr}
\Xhline{2\arrayrulewidth}
         & \multicolumn{1}{l}{PSNR} & \multicolumn{1}{l}{LPIPS} & \multicolumn{1}{l}{FID} & \multicolumn{1}{l}{Time} & \multicolumn{1}{l}{Param} \\ \hline\hline
Original & 0.00                     & 0.00                      & 0.00                    & 0.00                     & 0.00                      \\ \hline
Training-free     & 0.00                     & 0.00                      & 0.00                    & 0.00                     & 0.00                      \\
Depth 5 (FT)   & 0.00                     & 0.00                      & 0.00                    & 0.00                     & 0.00                      \\
Depth 4 (FT)   & 0.00                     & 0.00                      & 0.00                    & 0.00                     & 0.00                      \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}

\caption{\kkw{Qant StableSR depthSkip}}
\end{table}


==> tbls/_obsolete-skew.tex <==
\begin{table}[t]
\centering

\scalebox{0.9}{

\begin{tabular}{crcccc}

\Xhline{2\arrayrulewidth}
\multicolumn{1}{l}{Method} & \multicolumn{1}{c}{Steps} & Uniform & Skew   & $\gamma$ & Time (s) \\ \hline\hline
\multirow{5}{*}{IP2P}      & 5                         & 17.021  & 21.999 & 0.322 & 1846       \\
                           & 10                        & 23.086  & 25.856 & 0.556 & 1844       \\
                           & 15                        & 26.797  & 28.744 & 0.709 & 2227       \\
                           & 20                        & 29.705  & 31.372 & 0.769 & 2453       \\
                           & 25                        & 32.391  & 34.024 & 0.833 & 2577       \\ \hline
\multirow{5}{*}{StableSR}  & 5                         & 25.698  & 27.456 & 1.900 & 608        \\
                           & 10                        & 29.270  & 32.461 & 1.600 & 706        \\
                           & 15                        & 32.512  & 36.740 & 1.610 & 890        \\
                           & 20                        & 35.359  & 40.261 & 1.420 & 972        \\
                           & 25                        & 38.495  & 43.896 & 1.300 & 1028      \\
\Xhline{2\arrayrulewidth}

\end{tabular}

}
\caption{\kkw{skewed timesteps}}
\end{table}


==> tbls/autodiff-ip2p.tex <==
\begin{table}[t]
\centering
\caption{Quantitative comparison with AutoDiffusion for InstructPix2Pix~\cite{ip2p}.}

\scalebox{0.85}{

\begin{tabular}{cccl}
\Xhline{2\arrayrulewidth}
Method        & $\operatorname{CLIP}_{I}$ & $\operatorname{CLIP}_{D}$ & Search Time        \\ \hline\hline
Ours          & \textbf{0.767}            & \textbf{0.190}              & \textbf{38.7 min} \\
AutoDiffusion & 0.765                     & 0.188                       & 40.5 hour         \\ \Xhline{2\arrayrulewidth}
\end{tabular}

% \begin{tabular}{ccccc}
% \Xhline{2\arrayrulewidth}
% Method        & Layer-skip & Iteration & $\operatorname{CLIP}_{I}$ & $\operatorname{CLIP}_{dir}$ \\ \hline\hline
% Ours          &            & 5         & \textbf{0.767}            & \textbf{0.190}              \\
% AutoDiffusion &            & 5         & 0.765                     & 0.188                       \\
% AutoDiffusion & \checkmark & 5         & 0.765                     & 0.188                       \\ \hline
% Ours          &            & 10        & 0.763                     & \textbf{0.211}              \\
% AutoDiffusion &            & 10        & 0.764                     & 0.208                       \\
% AutoDiffusion & \checkmark & 10        & \textbf{0.765}            & 0.208                       \\ \Xhline{2\arrayrulewidth}
% \end{tabular}

% 5 step only version
% \begin{tabular}{cccc}
% \Xhline{2\arrayrulewidth}
% Method        & Layer-skip & $\operatorname{CLIP}_{I}$ & $\operatorname{CLIP}_{dir}$ \\ \hline\hline
% Ours          &            & \textbf{0.767}            & \textbf{0.190}              \\
% AutoDiffusion &            & 0.765                     & 0.188                       \\
% AutoDiffusion & \checkmark & 0.765                     & 0.188                       \\ \Xhline{2\arrayrulewidth}
% \end{tabular}


}
\label{tbl:autodiff-ip2p}
\vspace{+5mm}
\end{table}


==> tbls/autodiff-sdsr.tex <==

\begin{table}[t]
\centering
\caption{Quantitative comparison with AutoDiffusion for StableSR~\cite{stablesr}.}

\scalebox{0.85}{

\begin{tabular}{ccccl}
\Xhline{2\arrayrulewidth}
Method        & FID             & PSNR            & LPIPS          & Search Time        \\ \hline\hline
Ours          & \textbf{34.956} & 22.250          & \textbf{0.461} & \textbf{11.1 min} \\
AutoDiffusion & 36.496          & \textbf{22.347} & 0.466          & 27.1 hour          \\ \Xhline{2\arrayrulewidth}      
\end{tabular}

% \begin{tabular}{ccccc}
% \Xhline{2\arrayrulewidth}
% Method        & Layer-skip  & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$\\ \hline\hline
% Ours          &             & \textbf{34.956} & 22.250          & \textbf{0.461} \\
% AutoDiffusion &             & 36.496          & 22.347          & 0.466          \\
% AutoDiffusion & \checkmark  & 37.532          & \textbf{22.423} & 0.466          \\  \Xhline{2\arrayrulewidth}
% \end{tabular}

}
\label{tbl:autodiff-sdsr}
\end{table}


% \begin{table}[h]
% \centering

% \scalebox{0.85}{

% \begin{tabular}{ccccc}
% \Xhline{2\arrayrulewidth}
% Method        & Layer-skip  & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$\\ \hline\hline
% Ours          &             & \textbf{34.956} & 22.250          & \textbf{0.461} \\
% AutoDiffusion &             & 36.496          & 22.347          & 0.466          \\
% AutoDiffusion & \checkmark  & 37.532          & \textbf{22.423} & 0.466          \\  \Xhline{2\arrayrulewidth}
% \end{tabular}

% }
% \caption{Quantitative comparison with AutoDiffusion for StableSR~\cite{stablesr}. 10 iterations are used}
% \label{tbl:autodiff-sdsr}
% \end{table}


==> tbls/autodiff-time+time-quant.tex <==
\begin{table}[t]
    \centering
           \caption{
        Comparisons of search times for time-step optimization for each method. 
        }
        \scalebox{0.8}{
        \begin{tabular}{ccccccc}
        \Xhline{2\arrayrulewidth}
        
\multicolumn{1}{l}{} & \multicolumn{2}{c}{InstructPix2Pix~\cite{ip2p}} & \multicolumn{2}{c}{StableSR~\cite{stablesr}} & \multicolumn{2}{c}{ControlNet~\cite{controlnet}} \\
\multicolumn{1}{l}{} & 5 step     & 10 step     & 5 step       & 10 step       & 5 step        & 10 step        \\ \hline\hline
Xue et al.~\cite{xue2024accelerating}           & 3.2s       & 53.1s       & 3.2s         & 53.1s         & 3.2s          & 53.1s          \\
AutoDiffusion~\cite{autodiff}  & 40.5h      & 75.1h       & 16.3h        & 27.1h         & 31.2h         & 65.1h          \\
Ours                 & 38.7m      & 30.9m       & 9.5m         & 11.1m         & 14.4m         & 18.0m          \\
        \Xhline{2\arrayrulewidth}
    \end{tabular}    
    }
    \label{tbl:autodiff-time}
    \label{tab:my_label}
\end{table}


% \begin{table*}[t]
%     \begin{minipage}[b]{0.51\textwidth}

%         \centering
        
%         \caption{
%         Latency and MACs~\cite{thop} improvement after depth-skip pruning. 
%         % 50 iterations and RTX3090 GPU are used. 
%         }
%         \scalebox{0.63}{

% \begin{tabular}{ccccccc}
% \Xhline{2\arrayrulewidth}
% \multicolumn{1}{l}{} & \multicolumn{2}{c}{IP2P~\cite{ip2p}} & \multicolumn{2}{c}{StableSR~\cite{stablesr}} & \multicolumn{2}{c}{ControlNet~\cite{controlnet}} \\
% \multicolumn{1}{l}{} & Time(s)          & MACs(T)          & Time(s)       & MACs(T)      & Time(s)        & MACs(T)       \\ \hline\hline
% Original             & 6.312            & 50.81            & 2.807         & 18.75        & 1.572          & 18.21         \\
% D9                   & 5.978            & 47.27            & 2.421         & 17.49        & 1.444          & 17.26         \\
% D8                   & 5.685            & 41.75            & 2.204         & 15.57        & 1.372          & 15.79         \\
%         \Xhline{2\arrayrulewidth}

% \end{tabular}
        
        
%         }
%         \label{tbl:time-quant1}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.46\textwidth}

%         \raggedright 
%         \caption{
%         Time required for time-step search for each method. 
%         % Our method is significantly faster than AutoDiffusion~\cite{autodiff}.
%         }
%         \scalebox{0.63}{
        
%         \begin{tabular}{ccccccc}
%         \Xhline{2\arrayrulewidth}
        
% \multicolumn{1}{l}{} & \multicolumn{2}{c}{IP2P~\cite{ip2p}} & \multicolumn{2}{c}{StableSR~\cite{stablesr}} & \multicolumn{2}{c}{ControlNet~\cite{controlnet}} \\
% \multicolumn{1}{l}{} & 5 step     & 10 step     & 5 step       & 10 step       & 5 step        & 10 step        \\ \hline\hline
% Xue et al.           & 3.2s       & 53.1s       & 3.2s         & 53.1s         & 3.2s          & 53.1s          \\
% AutoDiffusion        & 40.5h      & 75.1h       & 16.3h        & 27.1h         & 31.2h         & 65.1h          \\
% Ours                 & 38.7m      & 30.9m       & 9.5m         & 11.1m         & 14.4m         & 18.0m          \\
%         \Xhline{2\arrayrulewidth}

% \end{tabular}
        
%         }
%         \label{tbl:autodiff-time}
    
%     \end{minipage}
%     \vspace{-4mm}
% \end{table*}

==> tbls/autodiff-time.tex <==
\begin{table}[t]
\centering 

\caption{
The time required for timestep optimization. 
Our method is significantly faster than AutoDiffusion~\cite{autodiff}.}

\scalebox{0.9}{

% \begin{tabular}{cccc}
% \Xhline{2\arrayrulewidth}
% \multicolumn{2}{c}{IP2P} & \multicolumn{2}{c}{StableSR} \\
% Ours    & AutoDiffusion  & Ours      & AutoDiffusion    \\ \hline\hline
% 30.9m   & 75.1h          & 11.1m     & 27.1h            \\ \Xhline{2\arrayrulewidth}
% \end{tabular}

\begin{tabular}{ccccc}

\Xhline{2\arrayrulewidth}
          & \multicolumn{2}{c}{IP2P}        & \multicolumn{2}{c}{StableSR}    \\
\textbf{} & 5 step         & 10 step         & 5 step          & 10 step         \\ \hline\hline
AutoDiffusion~\cite{autodiff}  & 40.5 h          & 75.1 h          & 16.3 h          & 27.1 h  \\
Ours             & \textbf{38.7 m} & \textbf{30.9 m} & \textbf{9.5 m} & \textbf{11.1 m}\\ 
\Xhline{2\arrayrulewidth}

\end{tabular}

}
\vspace{-3.0mm}
\label{tbl:autodiff-time}
\end{table}




==> tbls/controlnet.tex <==
\begin{table}[t]
\centering
\caption{
Quantitative comparisons of depth-skip pruning and other pruning methods for ControlNet~\cite{controlnet}.
}

% \scalebox{0.84}{
\scalebox{0.7}{
\begin{tabular}{lcccccc}
\Xhline{2\arrayrulewidth}
Model                                       & Fine-tune  & Steps & FID $\downarrow$  & CLIP-Score$\uparrow$ & CLIP-a$\uparrow$ & Param(\%) \\ \hline\hline
Diff-pruning~\cite{diffpruning}              & O          & 20    & 28.52             & 28.91          & 5.01             & 80.2   \\
BK-SDM~\cite{bksdm}                          & O          & 20    & 29.66             & 29.08          & 4.87             & 67.2   \\
Depth-skip ($D$9)                            & X          & 20    & 21.18             & 30.29          & 5.93             & 60.8   \\ \hline
Depth-skip ($D$9)                            & O          & 20    & \textbf{17.64}    & \textbf{30.46} & \textbf{5.88}    & \textbf{60.8} \\
Depth-skip ($D$9) + Timestep optimization    & O          & 15    & 18.65            & 30.37           & 5.87             & 60.8   \\ \hline 
Original (Baseline)                          & O          & 20    & 17.52             & 30.57          & 5.91             & 100.0  \\
Original                                     & X          & 20    & 19.88             & 30.42          & 6.10             & 100.0  \\ 
\Xhline{2\arrayrulewidth}

\end{tabular}
}
\end{table}

==> tbls/sdsr-ds-quant.tex <==
\begin{table}[t]
\centering

\caption{
Quantitative comparisons of depth-skip pruning and other pruning methods for StableSR~\cite{stablesr}.
}
\vspace{-3mm}

\scalebox{0.7}{

\begin{tabular}{lcccccc}
\Xhline{2\arrayrulewidth}
Model                                     & Fine-tune   & Steps   & FID$\downarrow$  & PSNR$\uparrow$   & LPIPS$\downarrow$  & Parameter                   \\ \hline\hline
Diff-pruning~\cite{diffpruning}           & O           & 50      & 38.70            & 21.20            & 0.483              & 578M\space(62.4\%)          \\
BK-SDM~\cite{bksdm}                       & O           & 50      & 64.46            & 21.45            & 0.492              & 615M\space(67.2\%)          \\
Depth-skip ($D$9)                         & X           & 50      & \textbf{28.55}   & \textbf{21.54}   & \textbf{0.441}     & \textbf{557M\space(60.8\%)} \\ \hline
Depth-skip ($D$8)                         & X           & 50      & 40.25            & 21.40            & 0.467              & 400M\space(43.6\%)          \\
Depth-skip ($D$8)                         & O           & 50      & \textbf{30.15}   & \textbf{21.48}   & \textbf{0.449}     & \textbf{400M\space(43.6\%)} \\ 
Depth-skip ($D$8) + Timestep optimization & O           & 20      & 32.31            & 21.82            & 0.457              & 400M\space(43.6\%)          \\ \hline
Original                                  & -           & 50      & 27.70            & 21.51            & 0.437              & 917M\space(100\%)           \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
}

\label{tbl:sdsr-ds-quant}
\vspace{-1mm}
\end{table}

==> tbls/sdsr-time-quant.tex <==
\begin{table}[t]

\centering
\scalebox{0.85}{

\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
Iteration    & 10             & 15             & 20             & 25             & 30             & 50                           \\ \hline\hline
Uniform & 38.50          & 35.31          & 33.08          & 32.20          & 31.41          & {\color[HTML]{1F1F1F} 30.15} \\
Ours    & \textbf{37.71} & \textbf{34.19} & \textbf{32.31} & \textbf{31.55} & \textbf{31.09} & -                            \\ \Xhline{2\arrayrulewidth}
\end{tabular}

}
  \caption{FID results using uniform and optimized timestep for StableSR~\cite{stablesr}. we achieve better metrics to various iterations.
  }
  \label{tbl:sdsr-time-quant}
\end{table}


==> tbls/sdsr-ts-quant.tex <==

\begin{table}[t]
\centering

\scalebox{0.85}{

\begin{tabular}{cccccccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l}{}   & Step    & 10            & 15            & 20            & 25            & 30            & 50   \\ \hline\hline
\multirow{2}{*}{FID$\downarrow$}   & Uniform & 35.7          & 32.5          & 30.4          & 29.3          & 28.4          & 27.7 \\
                       & Ours    & \textbf{35.0} & \textbf{31.5} & \textbf{29.6} & \textbf{28.6} & \textbf{28.0} & -    \\ \hline
\multirow{2}{*}{PSNR$\uparrow$}  & Uniform & \textbf{22.4} & \textbf{22.1} & \textbf{22.0} & \textbf{21.9} & 21.8          & 21.5 \\
                       & Ours    & 22.2          & 22.0          & 21.9          & 21.8          & 21.8          & -    \\ \hline
\multirow{2}{*}{LPIPS$\downarrow$} & Uniform & 0.46          & 0.45          & 0.45          & 0.44          & 0.44          & 0.44 \\
                       & Ours    & 0.46          & 0.45          & 0.45          & 0.44          & 0.44          & -    \\ \Xhline{2\arrayrulewidth}
\end{tabular}

}
\caption{Quantitative comparison on timestep optimization for StableSR~\cite{stablesr} }
\label{tbl:sdsr-ts-quant}
\end{table}


==> tbls/time-quant1.tex <==
\begin{table}[t]

\centering

\caption{
Latency and MACs~\cite{thop} improvement after depth-skip. 50 iterations and RTX3090 GPU are used.
}

\scalebox{0.9}{
\begin{tabular}{ccccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{InstructPix2Pix~\cite{ip2p}}  & \multicolumn{2}{c}{StableSR~\cite{bksdm}}                        \\
\multicolumn{1}{l}{} & \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{MACs(T)} & \multicolumn{1}{c}{Time(s)} & \multicolumn{1}{c}{MACs(T)} \\ \hline\hline
Original&   6.312    & 50.81  &   2.807  &  18.75    \\ \hline
$D$9    &   5.978    & 47.27  &   2.421  &  17.49     \\
$D$8    &   5.685    & 41.75  &   2.204  &  15.57    \\
%$D$7    &   5.383    & 36.48  &   2.001  &  13.72    \\
%$D$6    &   5.300    & 31.28  &   2.180  &  11.94    \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}

  \label{tbl:time-quant1}
  \vspace{-3mm}
\end{table}


==> tbls/time-quant2.tex <==
\begin{table}[t]

\centering
\scalebox{0.85}{

\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
       & \multicolumn{2}{c}{5 step} & \multicolumn{2}{c}{10 step} & \multicolumn{2}{c}{15 step} \\ 
Depth-skip &  -       & \checkmark  &     -      & \checkmark   &     -      & \checkmark     \\ \hline\hline
IP2P       & 0.322     & 0.322     & 0.556      & 0.556     & 0.709      & 0.714     \\
StableSR   & 1.900     & 1.900        & 1.600      & 1.600        & 1.610      & 1.610       \\
\Xhline{2\arrayrulewidth}
\end{tabular}

}
  \caption{Optimized $\gamma$ values with and without depth-skip compression for each iteration. The $\gamma$ values show minimal variation.}
  \label{tbl:time-quant2}
\end{table}

